Interval Decomposition of Persistence Modules over a Principal Ideal Domain

The study of persistent homology has contributed new insights and perspectives into a variety of interesting problems in science and engineering. Work in this domain relies on the result that any finitely-indexed persistence module of finite-dimensional vector spaces admits an interval decomposition -- that is, a decomposition as a direct sum of simpler components called interval modules. This result fails if we replace vector spaces with modules over more general coefficient rings. To address this problem, we introduce an algorithm to determine whether or not a persistence module of pointwise free and finitely-generated modules over a principal ideal domain (PID) splits as a direct sum of interval submodules. If one exists, our algorithm outputs an interval decomposition. When considering persistence modules with coefficients in $\Z$ or $\Q[x]$, our algorithm computes an interval decomposition in polynomial time. This is the first algorithm with these properties of which we are aware. We also show that a persistence module of pointwise free and finitely-generated modules over a PID splits as a direct sum of interval submodules if and only if the cokernel of every structure map is free. This result underpins the formulation of our algorithm. It also complements prior findings by Obayashi and Yoshiwaki regarding persistent homology, including a criterion for field independence and an algorithm to decompose persistence homology modules.

==> storage.tex <==
Topological data analysis (TDA) [cite things] is an area of data science that aims to capture and quantify the ``shape'' of data. One of the primary tools in TDA is persistent homology (PH) [cite things], which studies and quantifies holes in a data set. To perform PH on a data set, one first constructs a ``filtration,'' which is a nested sequence of topological spaces, that represent the aforementioned data set at different scales. PH studies how the homology --- which correspond to holes in the data --- changes in the filtration, from which one can infer topological structure of the data set in question. 
This information can be summarized by a ``persistence diagram'' [cite things]. 
PH has been used to study data in numerous areas, including biology [cite], images [cite], and geospatial analysis [cite]. 

PH is dependent upon the theory of persistence modules [cite], which are algebraic structures --- consisting of homology groups of a filtration --- that capture the homological information given by a filtration. Using field coefficients to take homology guarantees the existence of an ``interval decomposition'' for the persistence module, which provides the necessary information for computing the corresponding persistence diagram. 

Different choices of fields in computing homology may yield different interval decompositions, which in turn, yield different persistence diagrams. Additionally, when computing homology with non-field coefficients (e.g., integer coefficients), interval decompositions may not exist. In this paper, we provide the algebraic conditions for persistence modules under which persistence diagrams are independent of the choice of field. To do this, we study persistence modules of free abelian groups and provide the necessary and sufficient conditions under which interval decompositions exist. We additionally provide a polynomial-time algorithm to compute an interval decomposition for a persistence module of free abelian groups, when it exists. 
